Data Augmentation for Cross-Domain Named Entity Recognition

Current work in named entity recognition (NER) shows that data augmentation techniques can produce more robust models. However, most existing techniques focus on augmenting in-domain data in low-resource scenarios where annotated data is quite limited. In contrast, we study cross-domain data augmentation for the NER task. We investigate the possibility of leveraging data from high-resource domains by projecting it into the low-resource domains. Specifically, we propose a novel neural architecture to transform the data representation from a high-resource to a low-resource domain by learning the patterns (e.g. style, noise, abbreviations, etc.) in the text that differentiate them and a shared feature space where both domains are aligned. We experiment with diverse datasets and show that transforming the data to the low-resource domain representation achieves significant improvements over only using data from high-resource domains.

==> tables/ablation_study.tex <==
\begin{table}[H]
    \centering
    \small
    \renewcommand{\arraystretch}{1.2}
    \resizebox{0.8\linewidth}{!}{
        \begin{tabular}{l|cc}
            \toprule
            \bf Model & \bf Perplexity & \bf F1\\ 
            \toprule
            Full & 00.00 & 00.00 \\
            \toprule
            w/o noise injection & 00.00 & 00.00 \\
            $L_{adv}=0$         & 00.00 & 00.00 \\
            Teaching forcing = 1& 00.00 & 00.00 \\
            \toprule
        \end{tabular}
    }
    \caption{Ablation study. }
    \label{ref: ablation_study}
\end{table}

